A Derivational ChainBank for Modern Standard Arabic

We introduce the new concept of an Arabic Derivational Chain Bank CHAINBANK to leverage the relationship between form and meaning in modeling Arabic derivational morphology. We constructed a knowledge graph network of abstract patterns and their derivational relations and aligned it with the lemmas of the CAMELMORPH morphological analyzer database. This process produced chains of derived words' lemmas linked to their corresponding lemma bases through derivational relations, encompassing 23,333 derivational connections.

==> response.tex <==
R1:
Our  is not about morphological analysis, for which there are many existing tools as the reviewer points out. What we provide is a meta-level network that connects the different lexical items in terms of their derivational relationships. Most existing analyzers *do not* provide this information; and if they do, they indicate *flat* or *one-level* derivation. Our ChainBank can be used with all existing morphological databases. We will make sure to highlight this point in the paper.

Regarding the concern about rule-based systems, we agree; however what we are doing is creating a reference that can be used to train and/or evaluate ML/LLM models on the task of derivational relations.  This paper introduces the concept and demonstrates the feasibility of building it. 


R2:
Thanks for the comment and advice. We will clarify in the table and its caption that the 25/75 are numbers of roots not percentages. Following your advice, we will add more details on the performance by POS and relation type to elaborate on the reported results.


R3: 
Thanks for the comments and suggested edits. We will elaborate on the methodology with an extended example to highlight the benefits of the representation.








